On Graph Refutation for Relational Inclusions

We introduce a graphical refutation calculus for relational inclusions: it reduces establishing a relational inclusion to establishing that a graph constructed from it has empty extension. This sound and complete calculus is conceptually simpler and easier to use than the usual ones.

==> eptcsdata.tex <==
\providecommand{\firstpage}{47}
\providecommand{\publicationstatus}{Ronchi della Rocca, S., Pimentel, E. (Eds.): 6th Workshop
on\\ Logical and Semantic Frameworks with Applications 2011 (LSFA 2011).\\
EPTCS 81, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.81.4}{10.4204/EPTCS.81.4}}

